Efficient Computation of Optimal Trading Strategies

Given the return series for a set of instruments, a \emph{trading strategy} is a switching function that transfers wealth from one instrument to another at specified times. We present efficient algorithms for constructing (ex-post) trading strategies that are optimal with respect to the total return, the Sterling ratio and the Sharpe ratio. Such ex-post optimal strategies are useful analysis tools. They can be used to analyze the "profitability of a market" in terms of optimal trading; to develop benchmarks against which real trading can be compared; and, within an inductive framework, the optimal trades can be used to to teach learning systems (predictors) which are then used to identify future trading opportunities.

==> abstract.tex <==
Given the return series for a set of instruments,
a \emph{trading strategy} is a switching function that 
transfers wealth from one instrument to another at specified
times. We present efficient algorithms for constructing (ex-post)
trading strategies that are optimal with respect to the
total return, the Sterling ratio and 
the Sharpe ratio. Such ex-post 
optimal strategies  are useful analysis tools.
They can be used to analyze the ``profitability of a market'' in terms of
optimal trading; to develop 
benchmarks against which real trading can be compared; and,
within an inductive framework, the optimal trades can be used to
to teach learning systems (predictors) which are then used to identify 
future trading opportunities.   


==> conclusion.tex <==
\section{Discusion}

Our main goal was to provide the theoretical basis for the computation 
of \emph{a posteriori} optimal trading strategies, with respect to 
various criteria.
In particular, we have presented the algorithms, together
with the proofs of their correctness.
The highlights of our contributions are that return and sterling optimal
strategies can be computed very efficiently, even with constraints
on the number of trades. Sharpe optimal strategies prove to be much 
tougher to compute. However, for slightly modified notions of the
Sharpe ratio, where one ignores the impact of bid-ask spread squared
we can compute the optimal strategy efficiently. 
This is a reasonable approach since in most cases, the bid-ask spread 
is \math{\sim 10^{-4}}. We also show that this modified
optimal
strategy is not far from optimal with respect to the unmodified
Sharpe ratio.

Interesting topics of future research are to use these optimal strategies
to learn how to trade optimally, which was the original motivation of this 
work. Further, one could use them to benchmark trading strategies as well as
markets.
A natural open problem is whether Sharpe optimal strategies can be computed 
under constraints on the number of trades.
We suspect that the monotone hierarchy we created with respect to the
SSR has an important role to play, but the result has been elusive.

The algorithms presented here can be useful if one could relax Assumption
{\bf A1}. We have used such an assumption because it considerably 
simplifies the analysis, and in many cases, the optimal strategy is in fact
an all-or-nothing strategy.


At the core of some of our algorithms is a new technique for 
optimizing quotients over 
intervals of a sequence. 
This technique is based on relating the
problem to convex set operations, and for our purposes has
direct application to optimizing the \math{MDD}, the simplified Sharpe
ratio (SSR), 
which is an integral component in optimizing the Sharpe ratio, and
the Downside Deviation Ratio (DDR). This technique may be of more general
use in optimizing other financially important criteria.
As a result, such an algorithm may be of independent interest.



==> strl_overview.tex <==
\subsection{Overview of the Algorithm}

Based on the results in the previous section, the main observation is that 
if the Sterling optimal strategy makes two or more trades, then its
\math{MDD} will be the bid-ask spread, and hence it must be
the return optimal strategy. Thus we only need to consider the case when the
Sterling optimal strategy makes exactly one trade. A useful observatioin 
is that no optimal strategy will exit a trade in the middle of
a sequence of positive returns or enter a trade in the  middle of a 
sequence of negative returns. Thus the return sequence can be contracted
by combining any sequence of positive returns into a single
return, ans similarily any sequence of negative returns. Possible entry points
\math{a_i} correspond to the beginning of a positive return and 
exit points the end of a sequence of positive returns.

The main task is to find the Sterling optimal strategy making exactly one 
trade. We show that this problem can be reduced to convex hull operations
in 2-dimensions, and hence obtain an \math{O(n\log n)} algorithm for
constructing the optimal solution.

In order to construct the Sterling optimal strategy which makes at most
\math{K} trades, the basic idea is to start with the return optimal
strategy whose trade intervals
cannot be enlarged (maximal return optimal strategies). 
If this strategy makes at most \math{K} trades, then we are back to the 
unconstrained case. Otherwise, we show that one can successively merge 
neighboring trades in the return optimal strategy to obtain a 
sterling optimal strategy. The main difficulty in the algorithm is 
to determine which trades to merge, and we will show that a greedy 
merging strategy is in fact optimal.
